Tree decompositions and social graphs

Recent work has established that large informatics graphs such as social and information networks have non-trivial tree-like structure when viewed at moderate size scales. Here, we present results from the first detailed empirical evaluation of the use of tree decomposition (TD) heuristics for structure identification and extraction in social graphs. Although TDs have historically been used in structural graph theory and scientific computing, we show that---even with existing TD heuristics developed for those very different areas---TD methods can identify interesting structure in a wide range of realistic informatics graphs. Our main contributions are the following: we show that TD methods can identify structures that correlate strongly with the core-periphery structure of realistic networks, even when using simple greedy heuristics; we show that the peripheral bags of these TDs correlate well with low-conductance communities (when they exist) found using local spectral computations; and we show that several types of large-scale "ground-truth" communities, defined by demographic metadata on the nodes of the network, are well-localized in the large-scale and/or peripheral structures of the TDs. Our other main contributions are the following: we provide detailed empirical results for TD heuristics on toy and synthetic networks to establish a baseline to understand better the behavior of the heuristics on more complex real-world networks; and we prove a theorem providing formal justification for the intuition that the only two impediments to low-distortion hyperbolic embedding are high tree-width and long geodesic cycles. Our results suggest future directions for improved TD heuristics that are more appropriate for realistic social graphs.

==> header_BlairPf_fromBS.tex <==

% STOC submission header
\usepackage[margin=1in]{geometry}
\usepackage[latin2]{inputenc}
\usepackage[english]{babel}
\usepackage[all=normal,paragraphs=tight]{savetrees}
\usepackage{tikz}
%\usepackage{url}

\usepackage{graphicx}
%\usepackage{caption}
%\usepackage{subcaption}

%\usepackage[T1]{fontenc}
%\usepackage[latin1]{inputenc}

%\usepackage[notref]{showkeys} % Use option 'final' to remove

\usepackage{multicol}

% FONTS and SYMBOLS
\usepackage{bbm}
\usepackage{mathrsfs}
\usepackage{latexsym}
\usepackage{lmodern}

% MATHEMATICS
\usepackage{amsmath,amsfonts,amssymb,amsthm} % AMS packages
%\usepackage[warning, all]{onlyamsmath}
\usepackage{mathtools}
\usepackage{thmtools}
\usepackage{thm-restate}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{observation}[theorem]{Observation}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newcommand{\retheorem}{theorem}

% COLORS and GRAPHICS
%\usepackage[usenames,dvipsnames,table]{xcolor}
\usepackage{graphicx}

% FIGURES and TABLES
\usepackage{wrapfig}
\usepackage{booktabs} % Better tables
\usepackage{longtable}
\usepackage{float}

\usepackage{enumerate}
\usepackage{enumitem}
\usepackage{xspace}
\usepackage{comment}
\usepackage{ifthen}
\usepackage[noadjust,nospace]{cite} % Sort citations.
\usepackage{ellipsis}
\usepackage{fixltx2e}
\usepackage{url}
\usepackage{scrtime}

\usepackage{microtype} % Prettifies pdf output. Uncomment if you have trouble with this. Will also reduce page count.

\usepackage[ruled,longend,vlined,linesnumbered]{algorithm2e}

% MARGIN NOTES
\usepackage[draft,author=]{fixme}
\fxsetup{theme=color}
\newcommand{\todo}[1]{\fxerror{#1}}
\newcommand{\warn}[1]{\fxwarning{#1}}
\newcommand{\note}[1]{\fxnote{#1}}

%\usepackage{hyperref} % needs to be here, resolves conflicts with other
                      % packages (e.g.AMS)


\newcommand{\subexp}{\textsc{subexp}}
\newcommand{\dtime}[1]{\ensuremath{\mathsc{DTIME}(#1)}}
\newcommand{\subexpsubexp}[1]{\ensuremath{\mbox{\sc DTIME}(2^{o(#1)})/\mbox{\sc SubEXP}}}
\newcommand{\PP}{\ensuremath{\text{P}}\xspace}
% \newcommand{\NP}{\ensuremath{\text{NP}}\xspace}
\newcommand{\XP}{\ensuremath{\text{XP}}\xspace}
\newcommand{\FPT}{\ensuremath{\text{FPT}}\xspace}
\newcommand{\MCa}[2]{\ensuremath{\text{MC}(#1,#2)}}
\newcommand{\MC}[1]{\MCa{#1}{\cC}}
\newcommand{\MS}{\ensuremath{\text{MSO}}\xspace}
\newcommand{\MSO}{\ensuremath{\text{MSO}_1}\xspace}
\newcommand{\MSOii}{\ensuremath{\text{MSO}_2}\xspace}
\newcommand{\MSOL}{\ensuremath{\text{MSO_1\text{-}}L}\xspace}
\newcommand{\EMSO}{\ensuremath{\text{EMSO}}\xspace}
\newcommand{\PH}{\ensuremath{\text{PH}}\xspace}
\newcommand{\Tlarge}{\ensuremath{\mathcal{T}_{\text{large}}}}
\newcommand{\Tsmall}{\ensuremath{\mathcal{T}_{\text{small}}}}
\newcommand{\W}[1]{\ensuremath{\text{W}[#1]}}
\newcommand{\Wcomplete}[1]{\ensuremath{\text{W}$[#1]$-complete}}
\newcommand{\Whard}[1]{\ensuremath{\text{W}[#1]\text{-hard}}}
\newcommand{\PVD}{\textsc{$\mathcal P$-Vertex Deletion}}
\newcommand{\NPhard}{\ensuremath{\text{NP-hard}\xspace}}
\newcommand{\adj}{\ensuremath{\mathbf{adj}}\xspace}
\newcommand{\inc}{\ensuremath{\mathbf{inc}}\xspace}
\newcommand{\arc}{\ensuremath{\mathbf{arc}}\xspace}
\newcommand{\contract}{\ensuremath{\preceq_{\mathit{c}}}}

\newcommand{\N}{\ensuremath{\mathbf{N}}\xspace} % Natural numbers
\newcommand{\R}{\ensuremath{\mathbf{R}}\xspace}	% Real numbers
\renewcommand{\cal}{\mathcal}

\newtheorem*{mainI}{Theorem~I}{\bfseries \upshape}{\itshape}
\newtheorem*{mainII}{Theorem~II}{\bfseries \upshape}{\itshape}

\newcommand{\name}[1]{\textsc{#1}}
\newcommand{\rem}[1]{\textcolor{red}{[#1]}}
\newcommand{\modif}[1]{\textcolor{blue}{#1}}
\newcommand{\xtof}[1]{\textcolor{blue}{[Xtof: #1]}}
\newcommand{\epd}{extended $\omega$-protrusion decomposition}
\newcommand{\pd}{$(\alpha,\beta)$-protrusion decomposition}
\newcommand{\kpd}{$(\bigO(k),\beta)$-protrusion decomposition}
\newcommand{\pmincmso}{\name{$p$-min-CMSO}}
\newcommand{\pmaxcmso}{\name{$p$-max-CMSO}}
\newcommand{\peqcmso}{\name{$p$-eq-CMSO}}
\newcommand{\YES}{\textsc{yes}}
\newcommand{\NO}{\textsc{no}}
\newcommand{\Ex}{\mathop{\bf E\/}}
\newcommand{\mc}{\mathcal}
\newcommand{\mb}{\mathbf}
\newcommand{\mbb}{\mathbb}
%\newcommand{\qed}{\hfill $\Box$}
\newcommand{\M}{\mathcal{M}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\ov}{\overrightarrow}
\newcommand{\bigO}{\mathcal{O}}

\newcommand{\HC}{\textsc{$H$-Minor Cover}}
\newcommand{\dHC}{\textsc{Disjoint $H$-Minor Cover}}
\newcommand{\cHC}{\textsc{Colored $H$-Minor Cover}}
\newcommand{\acHC}{\textsc{Annotated  \& Colored $H$-Minor Cover}}
\newcommand{\planarF}{\textsc{Planar-$\mc{F}$-Deletion}}
\newcommand{\DplanarF}{\textsc{Disjoint Planar-$\mc{F}$-Deletion}}

\newenvironment{proofof}{\noindent \textit{Proof of claim. }}{\hfill$\Diamond$}
\newenvironment{reminder}[1]{\smallskip
\noindent {\bf Reminder of #1  }\em}{}
\newcommand{\Problem}[1]{\textsc{#1}\xspace}
\newcommand{\VC}{\Problem{Vertex Cover}}
\newcommand{\LongP}{\Problem{Longest Path}}
\newcommand{\ExP}{\Problem{Exact $k$-Path}}
\newcommand{\HamP}{\Problem{Hamiltonian Path}}
\newcommand{\DS}{\Problem{Dominating Set}}
\newcommand{\IM}{\Problem{Induced Matching}}
\newcommand{\FDST}{\Problem{Full-Degree Spanning Tree}}
\newcommand{\CP}{\Problem{Cycle Packing}}
\newcommand{\FVS}{\Problem{Feedback Vertex Set}}
\newcommand{\EDS}{\Problem{Edge Dominating Set}}
\newcommand{\CVD}{\Problem{Chordal Vertex Deletion}}
\newcommand{\TWtVD}{\Problem{Treewidth-$t$\- Vertex\- Deletion}}
\newcommand{\ClVD}{\Problem{Cluster Vertex Deletion}}
\newcommand{\IVD}{\Problem{Interval Vertex Deletion}}
\newcommand{\CoVD}{\Problem{Cograph Vertex Deletion}}
\newcommand{\ConnVC}{\Problem{Connected Vertex Cover}}
\newcommand{\ConnDS}{\Problem{Connected Dominating Set}}
\newcommand{\ConnClVD}{\Problem{Connected Cluster Vertex Deletion}}
\newcommand{\ConnCoVD}{\Problem{Connected Cograph Vertex Deletion}}

\newcommand{\NP}{\ensuremath{\text{NP}}\xspace}
\newcommand{\coNP}{\ensuremath{\text{co-NP}}\xspace}
\newcommand{\diam}{\ensuremath{\mathop{diam}}\nolimits} % Graph diameter
\newcommand{\minor}{\ensuremath{\preceq_{{\mathit{m}}}\!}} % Minor relation
\newcommand{\tminor}{\ensuremath{\preceq_{\mathit{tm}}\!}} % Top. minor relation

\DeclareMathOperator{\wcol}{wcol}
\DeclareMathOperator{\col}{col}
\DeclareMathOperator{\coim}{coim}

\DeclareMathOperator{\rad}{radius} % radius
\DeclareMathOperator{\den}{density} % density
\DeclareMathOperator{\avg}{avg} % average degree

%\newcommand{\wcol}{\ensuremath{\mathop{wcol}}\nolimits} % Weak coloring number
%\newcommand{\col}{\ensuremath{\mathop{col}}\nolimits} % Coloring number
%\newcommand{\coim}{\ensuremath{\mathop{coim}}}

\newcommand{\lexprod}{\ensuremath{\mathbin{{}\bullet{}}}}


\def\dir#1{\vec{#1}}
\def\grad_#1{\nabla\!_{#1}}
\def\topgrad_#1{\widetilde \nabla\!_#1}

\newcommand{\notminor}{\ensuremath{\npreceq_{{\mathit{m}}}\!}}
\newcommand{\nottminor}{\ensuremath{\npreceq_{{\mathit{tm}}}\!}}
\newcommand{\set}[1]{\ensuremath{\left\{#1\right\}}}
\newcommand{\poly}{\mathop\mathit{poly}}
\newcommand{\cliques}{\mathop{cliques}}  % Set of all cliques
\newcommand{\bound}{\ensuremath{\mathop{bd}}}    % Boundary symbol for t-boundaried graphs
\newcommand{\equipi}[1]{\ensuremath{\equiv_{\Pi,#1}}} % Equivalence for t-boundaried graphs with t as parameter
\newcommand{\prot}{\ensuremath{\rho}}   % Prot. repr. size
\newcommand{\protd}{\ensuremath{\rho'}} % Prot. repr. size with doubled parameter
\newcommand{\YYYY}{\ensuremath{Y_0 \uplus Y_1 \uplus \cdots \uplus Y_\ell}\xspace} % I don't want to type this anymore
\newcommand{\primedYYYY}{\ensuremath{Y_0' \uplus Y_1' \uplus \cdots \uplus Y_\ell'}\xspace} % Use this for a primed version of the decomposition 
\renewcommand{\le}{\leqslant}
\renewcommand{\leq}{\leqslant}
\renewcommand{\ge}{\geqslant}
\renewcommand{\geq}{\geqslant}

\newcommand{\widthm}[1]{\ensuremath{\mathop\mathbf{#1}}\xspace}
\newcommand{\tw}{\widthm{tw}}
\newcommand{\pw}{\widthm{pw}}
\newcommand{\td}{\widthm{td}}
\newcommand{\width}{\widthm{width}}
\newcommand{\cw}{\widthm{cw}}
\newcommand{\rw}{\widthm{rw}}
\newcommand{\treedecomp}{\ensuremath{\mathcal{T}}}
\newcommand{\degav}{\ensuremath{d_{avg}}}
\newcommand{\fii}{finite integer index\xspace} % Is shortened to FII in short.tex
\newcommand{\probvec}{\mathbf{x}} %%feel free to change this
\newcommand{\probpar}{\xi} %%feel free to change; used Greek instead of Latin since most of the latter are used for various purposes. 
\newcommand{\nab}{\mathop{\triangledown}}
\newcommand{\topnab}{\mathop{\tilde \triangledown}}
\newcommand{\FII}{FII\xspace} % Is shortened to FII in short.tex
\newcommand{\dist}{\ensuremath{\text{dist}}}
\newcommand{\clos}{\ensuremath{\text{clos}}}
\newcommand{\numcliques}{\ensuremath{\mathop{\#\omega}}}
%%%Ancestors and Descendants--These are sets and hence Capitals!%%%
\newcommand{\anc}[2]{\ensuremath{\text{Anc}_{#1}(#2)}}
\newcommand{\des}[2]{\ensuremath{\text{Des}_{#1}(#2)}}
\newcommand{\child}[2]{\ensuremath{\text{Children}_{#1}(#2)}}
\DeclareMathOperator{\degree}{deg}

\newcommand{\intro}{\ensuremath{\mathit{intro}}}
\newcommand{\forget}{\ensuremath{\mathit{forget}}}
\newcommand{\join}{\ensuremath{\mathit{join}}}

%\newtheorem{lemma}{Lemma}
%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}
%\newtheorem{observation}{Observation}
%\newtheorem{proposition}{Proposition}
%\newtheorem*{claim}{Claim}
%\newtheorem*{prob}{Problem}

%\theoremstyle{definition}
%\newtheorem{redrule}{Reduction Rule}
%\newtheorem{definition}{Definition}

% Abbreviations, typographically correct
\newcommand*{\eg}{e.g.\@\xspace}
\newcommand*{\ie}{i.e.\@\xspace}
\newcommand*{\cf}{cf.\@\xspace}
\newcommand*{\wrt}{w.r.t.\@\xspace}
\makeatletter
\newcommand*{\etc}{%
    \@ifnextchar{.}%
        {etc}%
        {etc.\@\xspace}%
}
\makeatother
\newcommand{\ditto}{\textbf{-- \raisebox{-3pt}{''} --}}%

%notes, todo, remarks
\newcommand\Color[2]{\textcolor{#1}{#2}}
\newcommand{\nb}[1]{\marginpar{\scriptsize #1}}
% \newcommand\todo[1]{\nb{\Color{red}{#1}}}
% \newcommand\todo[1]{[\Color{red}{#1}]}

% Short vs. long version commands:
\newif\ifshort
\newcommand{\short}[1]{%
    \ifshort%
        #1\fi%
}
\newif\ifappend
\newcommand{\append}[1]{%
    \ifappend%
        #1\fi%
}
\newcommand{\journal}[1]{%
    \ifshort%
    \else%
        #1\fi%
}
\newcommand{\omitted}{%
    \ifappend%
    \else%
        \textup{[$\star$]}
    \fi
}

\def\reduce{}
\def\Reduce{}
\def\REDUCE{}

\usepackage{framed}
\usepackage{ctable}
\newenvironment{problem}[1]{\ignorespaces%
                \begin{framed}%
                \begin{tabular*}{\textwidth}{@{\hspace{1em}} >{\itshape}l p{0.68\textwidth} @{}}%
                \multicolumn{2}{l}{\hspace{0.55em}\textsc{#1}} \vspace{.2em}\\
            }{
                \end{tabular*}%
                \end{framed}%
                \smallskip%
                \ignorespacesafterend%
             }

\newenvironment{defproblem}[1]{\noindent\ignorespaces%
                                \FrameSep=6pt%
                                \parindent=0pt%
                \begin{framed}%
                \begin{tabular*}{\textwidth}{@{\hspace{.1em}} >{\itshape} p{2cm} p{0.8\textwidth} @{}}%
                \multicolumn{2}{l}{\textsc{#1}} \vspace{.2em}\\
            }{
                \end{tabular*}%
                \end{framed}%
                \smallskip%
                \ignorespacesafterend%
             }

\usepackage{xargs}
\usepackage{framed}
\renewenvironmentx{leftbar}[2][1=0.5pt, 2=5pt]{% 
  \def\FrameCommand{\vrule width #1 \hspace{#2}}\MakeFramed {\advance\hsize-\width \FrameRestore}}%
{\endMakeFramed}
\newenvironment{draft}[1]{%
                \color{gray}%
                \begin{leftbar}%                
                \begin{center}\emph{Draft:} {#1}\end{center}
            }{
                \end{leftbar}%
             }

\newcommand{\roottdd}{\textup{td-r}}
\newcommand{\longpath}{\textup{LP}}
% \newcommand{\compxy}{\textup{COM}} 
\def\compxy(#1){\mathcal{U}_{#1}}

% Hard-to-type names and words
\def\Nesetril{Ne\v{s}et\v{r}il\xspace}
\def\Dvorak{Dvo\v{r}\'{a}k\xspace}
\def\Kral{Kr\'{a}l\xspace}
\def\supf{superfluous\xspace}


% Commands from notes. Should be replaced.

\newcommand{\alg}{{\mathbb{A}}}
\newcommand{\eps}{{\varepsilon}}
\newcommand{\Ss}{{\mathcal{S}}}
\newcommand{\height}{{\mathbf{height}}}
\newcommand{\cc}{{\mathcal{C}}}
\newcommand{\Oh}{{\mathcal{O}}}
\newcommand{\Ohstar}{{\mathcal{O}^*}}
\newcommand{\n}{{\mathbf{n}}}
\newcommand{\bla}{\nabla}
\newcommand{\ds}{\mathbf{ds}}
\newcommand{\Kappa}{K}

% Functions needed in the paper. Change names
% later.
\def\domcoresize{f_{\text{coresize}}}
\def\twinclassbound{f_{\text{twins}}}

